(Un)ranking Permutation Classes

Permutations avoiding a pattern of length three are enumerated by the Catalan numbers. In this work, we present methods for ranking and unranking such permutations in lexicographic or colexicographic order.

==> eptcsdata.tex <==
\providecommand{\firstpage}{114}
\providecommand{\publicationstatus}{S. Brlek and L. Ferrari (Eds.): GASCom 2026\\
EPTCS 445, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.445.14}{10.4204/EPTCS.445.14}}
\pdfoutput=1

